Attention-based Convolutional Autoencoders for 3D-Variational Data Assimilation

We propose a new 'Bi-Reduced Space' approach to solving 3D Variational Data Assimilation using Convolutional Autoencoders. We prove that our approach has the same solution as previous methods but has significantly lower computational complexity; in other words, we reduce the computational cost without affecting the data assimilation accuracy. We tested the new method with data from a real-world application: a pollution model of a site in Elephant and Castle, London and found that we could reduce the size of the background covariance matrix representation by O(10^3) and, at the same time, increase our data assimilation accuracy with respect to existing reduced space methods.

==> includes.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% University Assignment Title Page 
% LaTeX Template
% Version 1.0 (27/12/12)
%
% This template has been downloaded from:
% http://www.LaTeXTemplates.com
%
% Original author:
% WikiBooks (http://en.wikibooks.org/wiki/LaTeX/Title_Creation)
%
% License:
% CC BY-NC-SA 3.0 (http://creativecommons.org/licenses/by-nc-sa/3.0/)
% 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%----------------------------------------------------------------------------------------
%	PACKAGES AND OTHER DOCUMENT CONFIGURATIONS
%----------------------------------------------------------------------------------------
\usepackage[a4paper,hmargin=2.8cm,vmargin=2.0cm,includeheadfoot]{geometry}
\usepackage{textpos}
\usepackage{natbib} % for bibliography
\usepackage{tabularx,longtable,multirow,subfigure,caption}%hangcaption
\usepackage{fncylab} %formatting of labels
\usepackage{fancyhdr} % page layout
\usepackage{url} % URLs
\usepackage[english]{babel}
\usepackage{amsmath}
\usepackage{graphicx}
\usepackage{dsfont}
\usepackage{epstopdf} % automatically replace .eps with .pdf in graphics
\usepackage{backref} % needed for citations
\usepackage{array}
\usepackage{latexsym}
\usepackage[pdftex,pagebackref,hypertexnames=false,colorlinks]{hyperref} % provide links in pdf

\usepackage{listings}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareMathOperator*{\argmin}{arg\,min}
\usepackage{mathtools}


\hypersetup{pdftitle={Autoencoders for 3D-Variational Data Assimilation},
  pdfsubject={}, 
  pdfauthor={Julian Mack},
  pdfkeywords={Data Assimilation, Autoencoders, Variational, Background Covariance Matrix}, 
  pdfstartview=FitH,
  pdfpagemode={UseOutlines},% None, FullScreen, UseOutlines
  bookmarksnumbered=true, bookmarksopen=true, colorlinks,
    citecolor=black,%
    filecolor=black,%
    linkcolor=black,%
    urlcolor=black}

\usepackage[all]{hypcap}


%\usepackage{color}
%\usepackage[tight,ugly]{units}
%\usepackage{float}
%\usepackage{tcolorbox}
%\usepackage[colorinlistoftodos]{todonotes}
\usepackage{ntheorem}
\theoremstyle{break}
\newtheorem{lemma}{Lemma}

\usepackage{changepage}   % for the adjustwidth environment

\newenvironment{proof}{\begin{adjustwidth}{1cm}{1cm}}{\end{adjustwidth}}
  
% \newtheorem{theorem}{Theorem}
% \newtheorem{remark}{Remark}
% \newtheorem{definition}{Definition}
% \newtheorem{proof}{Proof}


%%% Default fonts
\renewcommand*{\rmdefault}{bch}
\renewcommand*{\ttdefault}{cmtt}



%%% Default settings (page layout)
\setlength{\parindent}{0em}  % indentation of paragraph

\setlength{\headheight}{14.5pt}
\pagestyle{fancy}
\renewcommand{\chaptermark}[1]{\markboth{\chaptername\ \thechapter.\ #1}{}} 
\providecommand{\tabularnewline}{\\}

\fancyfoot[ER,OL]{\sffamily\textbf{\thepage}}%Page no. in the left on odd pages and on right on even pages
\fancyfoot[OC,EC]{\sffamily }
\renewcommand{\headrulewidth}{0.1pt}
\renewcommand{\footrulewidth}{0.1pt}
\captionsetup{margin=10pt,font=small,labelfont=bf}


%--- chapter heading

\def\@makechapterhead#1{%
  \vspace*{10\p@}%
  {\parindent \z@ \raggedright \sffamily
    \interlinepenalty\@M
    \Huge\bfseries \thechapter \space\space #1\par\nobreak
    \vskip 30\p@
  }}

%---chapter heading for \chapter*  
\def\@makeschapterhead#1{%
  \vspace*{10\p@}%
  {\parindent \z@ \raggedright
    \sffamily
    \interlinepenalty\@M
    \Huge \bfseries  #1\par\nobreak
    \vskip 30\p@
  }}

\allowdisplaybreaks

\usepackage[utf8]{inputenc}

% Default fixed font does not support bold face
\DeclareFixedFont{\ttb}{T1}{txtt}{bx}{n}{12} % for bold
\DeclareFixedFont{\ttm}{T1}{txtt}{m}{n}{12}  % for normal

% % Custom colors
% \usepackage{color}
% \definecolor{deepblue}{rgb}{0,0,0.5}
% \definecolor{deepred}{rgb}{0.6,0,0}
% \definecolor{deepgreen}{rgb}{0,0.5,0}

% \usepackage{listings}

% % Python style for highlighting
% \newcommand\pythonstyle{\lstset{
% language=Python,
% basicstyle=\ttm,
% otherkeywords={self},             % Add keywords here
% keywordstyle=\ttb\color{deepblue},
% emph={MyClass, NewLoaderClass, NewConfig ,__init__},          % Custom highlighting
% emphstyle=\ttb\color{deepred},    % Custom highlighting style
% stringstyle=\color{deepgreen},
% frame=tb,                         % Any extra options here
% showstringspaces=false            % 
% }}


% % Python environment
% \lstnewenvironment{python}[1][]
% {
% \pythonstyle
% \lstset{#1}
% }
% {}

% % Python for external files
% \newcommand\pythonexternal[2][]{{
% \pythonstyle
% \lstinputlisting[#1]{#2}}}

% % Python for inline
% \newcommand\pythoninline[1]{{\pythonstyle\lstinline!#1!}}


==> tables/ethics.tex <==

\begin{tabular}{p{9cm}c}
\toprule
 & \textbf{Yes or no} \\
\textbf{Section 1: HUMAN EMBRYOS/FOETUSES }&  \\
\midrule
Does your project involve Human Embryonic Stem Cells? & $\times$  \\
Does your project involve the use of human embryos?& $\times$  \\
Does your project involve the use of human foetal tissues / cells?& $\times$  \\
\midrule
\textbf{Section 2: HUMANS } &  \\
\midrule
Does your project involve human participants?& $\times$  \\
\midrule
\textbf{Section 3: HUMAN CELLS / TISSUES}  &  \\
\midrule
Does your project involve human cells or tissues? (Other than from “Human Embryos/Foetuses” i.e. Section 1)? & $\times$  \\
\midrule
\textbf{Section 4: PROTECTION OF PERSONAL DATA} &  \\
\midrule
Does your project involve personal data collection and/or processing?  & $\times$  \\
Does it involve the collection and/or processing of sensitive personal data (e.g. health, sexual lifestyle, ethnicity, political opinion, religious or philosophical conviction)?  & $\times$  \\
Does it involve processing of genetic information? & $\times$  \\
Does it involve tracking or observation of participants? It should be noted that this issue is not limited to surveillance or localization data. It also applies to Wan data such as IP address, MACs, cookies etc.& $\times$  \\
Does your project involve further processing of previously collected personal data (secondary use)? For example Does your project involve merging existing data sets?& $\times$  \\
\midrule
\textbf{Section 5: ANIMALS} &  \\
\midrule
Does your project involve animals?  & $\times$  \\
\midrule
\textbf{Section 6: DEVELOPING COUNTRIES} &  \\
\midrule
Does your project involve developing countries? & $\times$  \\
If your project involves low and/or lower-middle income countries, are any benefit-sharing actions planned?  & $\times$  \\
Could the situation in the country put the individuals taking part in the project at risk?  & $\times$  \\
\midrule
\textbf{Section 7: ENVIRONMENTAL PROTECTION AND SAFETY}
\midrule
&  \\
Does your project involve the use of elements that may cause harm to the environment, animals or plants?  & $\times$  \\
Does your project deal with endangered fauna and/or flora /protected areas?  & $\times$  \\
Does your project involve the use of elements that may cause harm to humans, including project staff?  & $\times$  \\
Does your project involve other harmful materials or equipment, e.g. high-powered laser systems?  & $\times$  \\
\midrule
\textbf{Section 8: DUAL USE} &  \\
\midrule
Does your project have the potential for military applications?& $\times$\\
Does your project have an exclusive civilian application focus?& $\times$  \\
Will your project use or produce goods or information that will require export licenses in accordance with legislation on dual use items? & $\times$  \\
Does your project affect current standards in military ethics – e.g., global ban on weapons of mass destruction, issues of proportionality, discrimination of combatants and accountability in drone and autonomous robotics developments, incendiary or laser weapons? & $\times$  \\
\midrule
\textbf{Section 9: MISUSE } &  \\
\midrule
Does your project have the potential for malevolent/criminal/terrorist abuse?& $\times$  \\
Does your project involve information on/or the use of biological-, chemical-, nuclear/radiological-security sensitive materials and explosives, and means of their delivery?& $\times$  \\
Does your project involve the development of technologies or the creation of information that could have severe negative impacts on human rights standards (e.g. privacy, stigmatization, discrimination), if misapplied?& $\times$  \\
Does your project have the potential for terrorist or criminal abuse e.g. infrastructural vulnerability studies, cybersecurity related project? & $\times$  \\
\midrule
\textbf{SECTION 10: LEGAL ISSUES} &  \\
\midrule
Will your project use or produce software for which there are copyright licensing implications?& \checkmark\\
Will your project use or produce goods or information for which there are data protection, or other legal implications?  & $\times$  \\
\midrule
\textbf{SECTION 11: OTHER ETHICS ISSUES}&  \\
\midrule
Are there any other ethics issues that should be taken into consideration?& $\times$ \\
\end{tabular}


==> tables/parrish_AE.tex <==
\begin{tabular}{lccc}
\toprule
\multicolumn{1}{c}{\textbf{Model }} & \textbf{DA MSE} & \textbf{ Excecution Time (s)} \\ \midrule
Ref MSE  & 1.0001 & -   \\ 
\midrule
TSVD, $\tau = 791$, $M = n$ & 0.09132 & 2.5009  \\
TSVD, $\tau = 32$, $M = 0.1n$ & 0.0923 & 0.3182 \\
TSVD, $\tau = 32$, $M = 0.01n$ & 0.1046 & 0.0481 \\
TSVD, $\tau = 32$, $M = 0.001n$ & 0.1403 &  \textbf{0.0410}\\
\midrule
Tucodec-NeXt  & \textbf{0.0787} & 0.0537  \\
\bottomrule
\end{tabular}

%TSVD, $\tau = 32$, $M = 25$ & 0.1769 &  0.036 \\
%TSVD, $\tau = 32$, $M = 2$ & 0.3613 &  0.033 \\
